Beep: Balancing Effectiveness and Efficiency when Finding Multivariate Patterns in Racket Sports

Modeling each hit as a multivariate event in racket sports and conducting sequential analysis aids in assessing player/team performance and identifying successful tactics for coaches and analysts. However, the complex correlations among multiple event attributes require pattern mining algorithms to be highly effective and efficient. This paper proposes Beep to discover meaningful multivariate patterns in racket sports. In particular, Beep introduces a new encoding scheme to discover patterns with correlations among multiple attributes and high-level tolerances of noise. Moreover, Beep applies an algorithm based on LSH (Locality-Sensitive Hashing) to accelerate summarizing patterns. We conducted a case study on a table tennis dataset and quantitative experiments on multi-scaled synthetic datasets to compare Beep with the SOTA multivariate pattern mining algorithm. Results showed that Beep can effectively discover patterns and noises to help analysts gain insights. Moreover, Beep was about five times faster than the SOTA algorithm.

==> archives/kdd2021/algorithms/a_candidate.tex <==
\begin{algorithm}[t]
    \caption{Function for Candidate Patterns}
    \label{alg:candidate}
    \KwIn{A code table $CT$}
    \KwOut{A candidate code table $Cand$}
    \tcc{the explanation can be found in Sec. \ref{sec:candidates}}
    \For{{\bf each} $p_i \in CT$}{
        \For{{\bf each} $p_j \in CT$}{
            $Cand \leftarrow Cand \cup construct(p_i,~p_j)$\;
        }
    }
    \Return{$Cand$}
\end{algorithm}

==> archives/kdd2021/algorithms/a_covering.tex <==
\begin{algorithm}[t]
    \caption{Covering Algorithm}
    \label{alg:cover}
    \KwIn{A sequence $s$, a code table $CT$}
    \KwOut{An optimal cover $C$}
    \tcc{the explanation can be found in Sec. \ref{sec:coverAlgorithm}}
    $C \leftarrow \emptyset$, $marks \leftarrow \emptyset$, $misses \leftarrow \emptyset$\;
    \For{{\bf each} $p\in CT^*$ in Cover Order} {
        \For{{\bf each} $(marks\_p, misses\_p) \in search(p, s)$}{
            \If{$marks \cap marks\_p = \emptyset$}{
                $C \leftarrow C \cup (marks\_p, misses\_p)$\;
                $marks \leftarrow marks \cup marks\_p$\;
                $misses \leftarrow misses \cup misses\_p$\;
            }
        }
        \If{$|marks| = |s| \times |A|$}{
            {\bf break}\;
        }
    }
    \For{{\bf each} event $e \in s$} {
        \For{{\bf each} value $v \in e$} {
            \If{$v$ is not marked by $marks$} {
                $mark$ = \{cover $v$ by singleton pattern $v$ in $ST$\}\;
                $C \leftarrow C \cup (mark, \emptyset)$\;
                $marks \leftarrow marks \cup mark$\;
            }
        }
    }
    \Return{$C$}
\end{algorithm}

==> archives/kdd2021/algorithms/a_pruning.tex <==
\begin{algorithm}[t]
    \caption{Function for Pruning}
    \label{alg:pruning}
    \KwIn{The dataset $S$, a new pattern $p^*$, and a code table $CT$}
    \KwOut{A pruned code table $CT$}
    \tcc{the explanation can be found in Sec. \ref{sec:pruning}}
    $CT_p = CT \cup \{p^*\}$\;
    $PruneCand = \{p\in CT^*~|~usage(p~|~CT_p)<usage(p~|~CT)\}$\;
    \For{{\bf each} $p \in PruneCand$ in Prune Order}{
        \If{$L(S,~CT \setminus p) < L(S,~CT)$}{
            $CT \leftarrow CT \setminus p$\;
        }
    }
    \Return{$CT$}
\end{algorithm}

==> archives/kdd2021/algorithms/a_summarizing.tex <==
\begin{algorithm}[t]
    \caption{Summarizing Algorithm}
    \label{alg:summarizing}
    \KwIn{The dataset $S$ and the standard code table $ST$}
    \KwOut{An approximate optimal code table $CT$}
    \tcc{the explanation can be found in Sec. \ref{sec:summarizing}}
    $CT \leftarrow ST$\;
    $Cand \leftarrow candidate(CT)$\;
    \For{{\bf each} $p \in Cand$ in Candidate Order}{
        \If{$L(S,~CT \cup \{p\}) < L(S,~CT)$}{
            $CT \leftarrow prune(S,~p,~CT) \cup \{p\}$\;
            $CT \leftarrow variations(S,~p,~CT)$\;
            $Cand \leftarrow candidate(CT)$\;
        }
    }
    \Return{$CT$}
\end{algorithm}

==> archives/kdd2021/contents/0_0_title.tex <==
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
%%
%% If your title is lengthy, you must define a short version to be used
%% in the page headers, to prevent overlapping text. The \verb|title|
%% command has a ``short title'' parameter:
%% \begin{verbatim}
%%   \title[short title]{full title}
%% \end{verbatim}
\title{\textsc{Beep}: An Effective and Efficient Pattern Mining Algorithm\\for Multivariate Event Sequence Data}

==> archives/kdd2021/contents/0_1_authors.tex <==
%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Jiang Wu}
\email{wujiang5521@zju.edu.cn}
\affiliation{%
  \institution{Zhejiang Lab}
  \city{Hangzhou}
  \state{Zhejiang}
  \country{China}
}

\author{Dongyu Liu}
\email{dongyu@mit.edu}
\affiliation{%
  \institution{Massachusetts Institute of Technology}
  \city{Cambridge}
  \state{MA}
  \country{USA}
}

\author{Ziyang Guo}
\email{ziyangguo27@zju.edu.cn}
\affiliation{%
  \institution{Zhejiang University}
  \city{Hangzhou}
  \state{Zhejiang}
  \country{China}
}

\author{Yingcai Wu}
\authornote{Yingcai Wu is the corresponding author.}
\email{ycwu@zju.edu.cn}
\affiliation{%
  \institution{Zhejiang Lab}
  \city{Hangzhou}
  \state{Zhejiang}
  \country{China}
}

%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
% \renewcommand{\shortauthors}{Wu, et al.}

==> archives/kdd2021/contents/0_2_abstract.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
  Pattern mining is essential for the analysis of event sequence data.
  However, analysis of multivariate event sequence data, a common type of real-world data where each event includes multiple attributes, requires pattern mining algorithms to be highly effective and efficient.
  In this paper, we propose \textsc{Beep}, a novel algorithm that can efficiently discover a small set of meaningful patterns based on the Minimum Description Length principle.
  In particular, \textsc{Beep} introduces a new encoding scheme to discover patterns that can reveal correlations among multiple attributes and are highly tolerant of noise.
  Furthermore, \textsc{Beep} applies a tailored acceleration method based on Locality-Sensitive Hashing, which can greatly reduce the time for summarizing patterns.
  Empirical study on a real-world dataset shows that patterns discovered by \textsc{Beep} help analysts gain new and effective insights, while quantitative experiments on multi-scaled synthetic data show that our algorithm can discover these meaningful patterns about 5 times faster than the current state-of-art algorithm.
\end{abstract}

%dyu
% Identifying frequent sequential patterns among event sequence data is essential tasks in many disciplines.
% However, in real world, 

==> archives/kdd2021/contents/0_3_keywords.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003752.10003809.10010031.10010032</concept_id>
<concept_desc>Theory of computation~Pattern matching</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Theory of computation~Pattern matching}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{efficient algorithm, multivariate event sequence, MDL principle}

==> archives/kdd2021/contents/0_4_copyright.tex <==
%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
\setcopyright{acmcopyright}
\copyrightyear{2021}
\acmYear{2021}
% \acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
\acmConference[KDD '21]{KDD '21: ACM SIGKDD Conference on Knowledge Discovery and Data Mining}{August 14--18, 2021}{Singapore}
\acmBooktitle{KDD '21: ACM SIGKDD Conference on Knowledge Discovery and Data Mining, August 14--18, 2021, Singapore}
% \acmPrice{15.00}
% \acmISBN{978-1-4503-XXXX-X/18/06}

==> archives/kdd2021/contents/1_Introduction.tex <==
\section{Introduction}

\label{sec:Introduction}

Event sequence data -- i.e. data consisting of time-stamped or ordered events --- is widely used in many fields, including medical data analysis, sports data analysis, and consumer behavior analysis.
% Sequential data is widely used in many fields, including genetics, medical data analysis, sports data analysis, and consumer behavior analysis.
To better comprehend large sets of event sequences and obtain useful insights, analysts in these fields often use pattern mining algorithms~\cite{mabroukeh2010taxonomy,fournier2017survey} to discover and summarize patterns, i.e., the subsequences that occur frequently.

% multiple attributes bring two requirements
As information technology continues to progress, enabling the collection of more specific data, real-world event sequence data becomes more complex \cite{gan2018survey}.
% With the development of information technology in these fields, real-world event sequences data becomes more complex \cite{gan2018survey}.
For example, data produced during a table tennis game may now include the players' position, the ball's position, the technique used to hit, the spin direction of the ball, and more.
To work well with event sequences that include multiple attributes --- also known as multivariate event sequences --- pattern mining algorithms should be both \textbf{effective} and \textbf{efficient}.
% For example, to describe a hit event in tennis, we need to record the players' position, the ball's position, the technique used to hit, and the spin direction of the ball, et al.
% The multivariate event sequence data brings two requirements to current pattern mining algorithms: \textbf{effectiveness} and \textbf{efficiency}.

\textbf{Effective} pattern mining algorithms can discover patterns that reveal meaningful information about the sequences. To be effective, a pattern mining algorithm for multivariate event sequences must fulfill three conditions:
(1) The correlations among multiple attributes within sequences should be preserved for domain analysis.
For example, in table tennis, tactical patterns that reveal the players' playing style can involve multiple attributes.
One tactical pattern may be that when a player hits the ball to a certain \textit{position} on the table, the opponent always uses a specific \textit{technique} in response.
Univariate patterns cannot reveal the multivariate tactical patterns comprehensively.
% (1) It must be able to preserve correlations among multiple attributes within extracted patterns for domain analysis.
(2) The algorithm should have a high tolerance for single-value noises.
For example, in table tennis, when a player applies a tactical pattern, he/she may only change the technique of one hit to a similar technique, retaining the overall playing style.
We regard the changes on only one attribute as single-value noises, which should not prevent the algorithm from detecting the overall pattern.
% (2) The algorithm should have a high tolerance for noise data --- only one attribute is allowed to have a noise value in the data record.
% (2) It must have a high tolerance for noise data. Because noise is an essential problem in multivariate sequences, effective algorithms allow only one attribute that has a noise value in the data record.
(3) The number of returned patterns should be manageable. Given that multivariate patterns are complicated, analyzing them is time-consuming.
Only a small number of meaningful patterns should be returned to reduce the burden of analysis.
% (3) It must identify a manageable number of helpful patterns.

% Second, we need an efficient pattern mining algorithm that can summarize patterns within a few seconds.
% Second, we need an efficient pattern mining algorithm whose response time is acceptable---typically within a few seconds---for an interactive application.
% The outputs of a pattern mining algorithm eventually should be interpreted by human users.
% Thanks to the human eye's inherence to perceive information in parallel, visualization is a preferred way for analysts to explore multivariate event sequences~\cite{loorak2015timespan,wu2020visual}.
% Thanks to the human eye's inherence to perceive information in parallel, visualization is a preferred way for domain experts to explore multivariate sequential data~\cite{loorak2015timespan,wu2020visual}.
% In a visual analytics system, interactivity plays an essential role in supporting comprehensive data exploration.
% A pattern mining algorithm with high efficiency is the basis of seamless interactions.
\textbf{Efficient} pattern mining algorithms can mine multivariate patterns within an acceptable response time.
% Multivariate patterns may contain values of different attributes.
In a real-world scenario, the time allowed for pattern analysis is limited and cannot go forever.
Another scenario is that some parameters should be adjusted based on the analysts' feedback so that the patterns can satisfy the analysts' requirements.
In both scenarios, the algorithm is expected to return the results as soon as possible.
However, the multivariate patterns may contain values of different attributes, thus resulting in the huge search space of multivariate patterns.
A truly efficient algorithm is able to explore this huge, multivariate search space in a reasonable amount of time.

To the best of our knowledge, existing multivariate pattern mining algorithms cannot satisfy these two requirements simultaneously.
One set of traditional sequential pattern mining algorithms is based on thresholding \cite{fournier2017survey}. These algorithms tend to return an enormous number of patterns rather than seeking the most meaningful ones.
Some multivariate pattern mining algorithms \cite{morchen2007efficient,chen2010efficient,bertens2014characterising} transform multivariate sequences into univariate ones, such that extracted patterns cannot retain any correlations between attributes.
DITTO~\cite{bertens2016keeping} summarizes patterns with correlations between multiple attributes, but does not have high noise tolerance.

% our algorithm
In this paper, we propose \textsc{Beep}, a novel sequential pattern-mining algorithm which \textbf{B}alances \textbf{E}ffectiveness and \textbf{E}fficiency when finding \textbf{P}atterns.
Our algorithm is based on the Minimum Description Length (MDL) principle \cite{grunwald2007minimum}, chosen for its ability to summarize numerous sequences with a small number of informative patterns.
\textsc{Beep} considers a set of multivariate patterns as the model to preserve correlations among multiple attributes.
The main contributions of \textsc{Beep} consists of two parts.
First, for each pattern in the model, \textsc{Beep} introduces a new encoding scheme to encode the noise values in a dataset.
Second, to efficiently discover such an informative model, \textsc{Beep} applies a tailored acceleration method based on \textit{Locality Sensitive Hashing} so that the patterns with high frequencies can be found in a short time.
% \ldy{More description here about our algorithm to highlight what is novel here? What we have done to make the satisfaction of the two requirements possible?}

% evaluation
To evaluate the effectiveness of \textsc{Beep}, we worked with analysts to conduct an empirical study on a real-world dataset, namely the table tennis data.
Our tests show that \textsc{Beep} can mine a small number of informative multivariate patterns and handle noise well.
We conducted further quantitative experiments with synthetic datasets to compare \textsc{Beep} with the current state-of-art algorithm.
% To empirically evaluate our algorithm, we conduct experiments on both real-world datasets and synthetic datasets.
% Based on the results of the experiments, we further compare our algorithm with the state-of-art algorithms.
The results of the experiments prove that \textsc{Beep} can discover patterns that summarize the dataset better and save a great amount of time.

% organization of this paper
% We organize the rest of this paper as follows.
% We first define the data structure in Section \ref{sec:Predefinitions} and briefly introduce the MDL principle in Section \ref{sec:MDL}.
% Then, we illustrate our algorithm in detail in Section \ref{sec:F4M} and discuss related work in Section \ref{sec:RelatedWork}.
% Furthermore, we evaluate our algorithm in Section \ref{sec:Experiments}.
% Finally, we discuss and conclude our work in Section \ref{sec:Discussion} and Section \ref{sec:Conclusion}, respectively.

==> archives/kdd2021/contents/2_Predefinitions.tex <==
\section{Definitions}

\label{sec:Predefinitions}

In this section, we formally define the input and the output of \textsc{Beep}.

\textbf{Input: }
We define the input as a dataset $S$ of multivariate event sequences, where the number of sequences is denoted by $|S|$.
% We consider a dataset $S$ of $|S|$ multivariate event sequences as the input of our algorithm.
Each sequence $s_i \in S$ is a vector of $|s_i|$ events, denoted $s_i = (e_1, e_2, ..., e_{|s_i|})$.
We further define $||S||=\sum_i{|s_i|}$ as the number of events in the whole dataset.
For each event $e$, we consider a same set of categorical attributes $A=\{a_1, a_2, ..., a_{|A|}\}$.
Thus, an event $e$ can be considered a vector of values, denoted $e=(v_1, v_2, ..., v_{|A|})$, where for each $1 \leq k \leq |A|$, $v_k$ is an optional value of attribute $a_k$.
We define $V_k$ as a finite set of all optional values of attribute $a_k$.
Thus, the set $E$ of all distinct events has a maximum size of $|E|_{max} = \prod_{1\leq k\leq |A|}{|V_k|}$.
% The dataset $S$ is over multiple categorical attributes $A=\{a_1, a_2,\\ ..., a_{|A|}\}$.
% Finite set $V_k$ consists of all the optional values for the $k$-th attribute $a_k$.
% Furthermore, an event $e$ can be considered as a vector of values, denoted $e=(v_1, v_2, ..., v_{|A|})$, where the $k$-th value $v_k \in V_k$.
% We define $E$ as the set of all distinct events, where the size $|E|$ has a maximum value of $|E|_{max} = \prod_{1\leq k\leq |A|}{|V_k|}$.

\textbf{Output: }
The output of \textsc{Beep} is a set $P$ of $|P|$ multivariate patterns. To define a pattern we must first define two other pre-elements.
First, we define $e^a\preceq e^b$ to indicate that event $e^a$ preserves some attributes of event $e^b$ and drops others, i.e., $e^a$ is part of $e^b$ (e.g., in Figure \ref{fig:patterndef}, $e_1$ of $p_1$, which drops the first attribute, is part of $e_1$ of $s_1$).
Formally, assume that $I$ is the set that includes the indexes of all the attributes to be preserved (i.e., some integers between 1 and $|A|$). For each $1\leq k\leq |A|$, if $k \in I$, $e^a$ has the same $k$-th value as $e^b$.
Otherwise, the $k$-th value of $e^a$ is empty.
Second, we define $s^a \subseteq s^b$ to indicate that sequence $s^a=(e^a_1, ..., e^a_n)$ is a subsequence of sequence $s_b=(e^b_1, ..., e^b_m)$, if there exist integers $1\leq i_1\le i_2\le ...\le i_n\leq m$ such that $e^a_j\preceq e^b_{i_j}$ for each $1\leq j\leq n$.

Based on these two pre-definitions, we define a pattern $p_i \in P$ as a subsequence of numerous original sequences in the dataset $S$, where $|p_i|$ indicates the length and $||p_i||$ indicates the number of values.
For example, in Figure \ref{fig:patterndef}, there exist four sequences ($s_1$ to $s_4$) in a dataset over two attributes ($a_1$ and $a_2$).
The dataset can be summarized by two patterns ($p_1$ and $p_2$), where $|p_1|=|p_2|=3$, $||p_1||=4$, and $||p_2||=6$.
Sequence $s_1$ covered by pattern $p_1$ is the simplest case.
We further support three features as follows to obtain informative patterns in real-world dataset.

\input{figures/patternDefinition}

\begin{enumerate}[label={\bf F{{\arabic*}}}]
  \item \label{feature:gap} \textbf{Gap events.}
%   A gap event can separate two consecutive events in the pattern into non-consecutive events in the sequence, such as $e_2$ of $s_2$.
  A gap event can separate two consecutive events in the pattern into non-consecutive events in the sequence. For example, sequence $s_2$ is covered by pattern $p_2$, but the gap event $e_2$ is not captured by $p_2$.
  We allow gaps to ignore events that may be noise.

  \item \label{feature:miss} \textbf{Missing values.}
  A missing value occurs in the pattern but not in the sequence, e.g., $s_3$ misses the second value of $e_2$ when it is covered by $p_2$.
  In the strictest interpretation, pattern $p_2$ is not a subsequence of sequence $s_3$.
  However, we must consider the possibility (common in real-world data) that a missing value is actually noise.
  Value $z$ may be similar to value $y$ because they have similar contexts (e.g., in tennis, $drive$ and $topspin$ are both offensive techniques to hit hard and low), or it may be an anomaly (e.g., an error caused by an automatic data acquisition system).
  Ignoring the substitution of similar values can keep the pattern simple, while detecting the pattern despite anomalies can help to inspect and dig into the data.
  Note that we are the first work that introduces missing values into multivariate sequential pattern mining.

  \item \label{feature:interleaveing} \textbf{Interleaving patterns.}
  Two interleaving patterns overlap over a period of time\cite{tatti2012long}, e.g., pattern $p_1$ and $p_2$ are interleaving in sequence $s_4$.
  We allow interleaving patterns to discover simultaneous patterns.
\end{enumerate}

An informative pattern should be compact (i.e., the events in the pattern should occur within a short period of time in the original sequences) and authentic (i.e., there should exist as few missing values as possible).
Thus, we limit the maximum number of gap events in a pattern $p$ to $|p|-1$ and the maximum number of missing values in a pattern $p$ to $\lfloor||p|| \div 10 + 0.5\rfloor$.
Moreover, we allow only one missing value in an event.


==> archives/kdd2021/contents/3_1_MDL.tex <==
\subsection{MDL principle}

The MDL principle was originally theorized in the context of data compression \cite{grunwald2007minimum}.
In order to minimize storage space, MDL describes the original dataset $D$ with a model $M$, which usually suggests the regularity in the data.
The MDL principle works under the assumption that the optimal model results in the shortest description length.
More formally, an optimal model $M$ can minimize $L(M) + L(D|M)$, where $L(M)$ is the description length of model $M$, and $L(D|M)$ is the description length of the original dataset $D$ when $D$ is described by $M$.
An MDL-based algorithm usually aims to solve three problems; namely, how to design a model, how to encode the dataset using a model, and how to obtain the optimal model.

In the past two decades, MDL has been applied to sequential pattern mining \cite{siebes2006item,tatti2012long,bertens2016keeping,kawabata2018streamscope}, and there exists a robust framework to solve the three problems mentioned above.
In our paper, we follow this framework and extend it to meet our requirements for effectiveness and efficiency.
Our solutions to the three aforementioned problems are as follows.
We define our model in Section \ref{sec:ct}, introduce the process of encoding in Section \ref{sec:encoding}, and propose our algorithm for obtaining model in Section \ref{sec:F4M}.
% Our solutions to the three questions are as follows.

==> archives/kdd2021/contents/3_2_CT.tex <==
\subsection{Code Table}

\label{sec:ct}

In prior work, code tables (\textit{CT}), which provide an encoding scheme for every pattern, have been widely used for model design.
We follow the design of code tables and further extend it to support two advanced features: gap events (\ref{feature:gap}) and missing values (\ref{feature:miss}).
As shown in Fig. \ref{fig:ct}, each row of a code table is associated with a pattern $p_i$, which is recorded in the first column.
To preserve the correlations between multiple attributes, the pattern can be multivariate.
The four columns on the right record four types of codes.
The second column records a pattern code $code_p(p_i)$ that represents the first event of the pattern, which indicates the occurrence of the pattern.
The gap code $code_g(p_i)$ (the third column) and the fill code $code_f(p_i)$ (the fourth column) support the gap events feature.
The two codes are introduced and well evaluated in prior works \cite{tatti2012long, bertens2016keeping}.
A gap code represents a gap event in the sequence, and a fill code represents an event in the pattern to be filled in the sequence (with the exception of the first event represented by the pattern code).

We propose a new code (the fifth column), namely the miss code $code_m(p_i)$, to allow for the missing values feature \ref{feature:miss}.
A miss code is a number to indicate the index of the missing value.
After an event is encoded by a pattern code or a fill code, there may exist a miss code to show which attribute of the event is missing.

When we implement the code table, two more constraints arise.
First, following our limitations on gap events and missing values, for a pattern $p_i$, the number of the gap code must be smaller than $|p_i|$, the number of the fill code must be $|p_i| - 1$, and the number of the missing code must be smaller than $\lfloor||p_i|| \div 10 + 0.5\rfloor$.
Given these limitations, we find it useless to record the gap code and the fill code for a pattern $p$ that satisfies $|p| = 1$ and to record the miss code for a pattern $p$ that satisfies $||p|| < 5$.
Thus, we delete these useless codes to shorten the description length.

Second, to ensure that a sequence can be completely covered by the model, we further extend $CT$ with all singleton values, which are regarded as patterns with only one value.
The extended rows are regarded as the standard code table ($ST$) because it is the minimum $CT$.
Obviously, the patterns in $ST$ cannot deliver insight into the sequences.
To distinguish the informative patterns with more than one value from these singleton patterns, we define $CT^*$ as the table of all the patterns in $CT$ but not in $ST$.
The output of our algorithm is all the patterns in $CT^*$.

\input{figures/encoding}

==> archives/kdd2021/contents/3_3_Encoding.tex <==
\subsection{Dataset Encoding}

\label{sec:encoding}

To encode the dataset with the code table, our algorithm takes three steps: covering, encoding, and calculating the encoded length.

\subsubsection{Covering}

Covering is the process of using patterns to describe a sequence.
A sequence $s$ is first separated into several patterns in code table $CT$ without overlapped values. The result is called a cover $C=cover(s~|~CT)$.
In the formal manner, given a sequence $s$ and a code table $CT$, a cover $C$ records which patterns are used and the location of each value in the pattern.
For example, sequence $s$ in Fig. \ref{fig:ct} is covered by pattern $p_1$, pattern $p_2$ and singleton value $y$.
For pattern $p_1$, cover $C$ records that it covers the first three events, and that there exists one miss value at the second attribute of $e_2$, and no gap events.
For pattern $p_2$, cover $C$ records that it covers the events $e_2$, $e_4$, and $e_5$, and that there exists one gap event and no miss value.
For singleton value $y$, cover $C$ simply records its position.

Note that for a given code table, there may exist many ways of varying utility to cover a sequence.
The simplest way is to use only singleton values to cover the sequence.
However, this is also the least useful way, because it cannot compress any information or extract any patterns.
In section \ref{sec:coverAlgorithm}, we explain how \textsc{Beep} finds an optimal way to cover a sequence with our code table design.

\subsubsection{Encoding}

Encoding is the process of using codes in the code table to describe a sequence, rather than patterns.
Given a multivariate sequence $s$, a code table $CT$, and a cover $C$, we encode the sequence into a code stream $cs$ through four steps.
(1) Scan the sequence $s$ left-to-right and top-to-bottom to find the first value that is not encoded, and look up the pattern $p_i$ to which the value belongs in the cover $C$.
(2) Traverse the sequence $s$ from the first event of $p_i$ to the last event of $p_i$.
During the traversal, the first event of $p_i$ is encoded as the pattern code $code_p(p_i)$, the gap events are encoded as gap codes, and the other events are encoded as fill codes.
All these codes are sorted in the order they are traversed.
(3) Find all the miss values in cover $C$.
For each miss value, assuming that it belongs to event $e$, we insert the miss code after the pattern code or the fill code that encodes $e$.
(4) Concatenate the code stream of the pattern to the entire code stream and mark all the values in the pattern as encoded.
We repeat these four steps until all the values in the sequence are encoded.

For example, Fig. \ref{fig:ct} demonstrates how a sequence $s$ is encoded as a code stream $CS$ given a cover $C$ and a code table $CT$.
We encode $s$ with three patterns, namely, $p_1$, $p_2$, and singleton $y$, in the order of traversal.
We first encode $p_1$ with no gap events and a missing value at $a_2$ of $e_2$.
Then, we encode $p_2$ with one gap event and no missing values.
Finally, we encode the singleton value $y$.


\subsubsection{Calculating the Encoded Length}

After encoding, we need to calculate the encoded length of the dataset to evaluate the model.
We consider the encoded length in two parts, namely the encoded length of the code table $L(CT~|~C)$ and the encoded length of the dataset $L(S~|~CT)$.
The optimization goal is to minimize the total encoded length $L(CT~|~C)+L(S~|~CT)$.

As the basis, we consider the length of each code.
Given that each code should be unique in order to avoid ambiguity during decoding, we use prefix codes \cite{cover1999elements} to optimize the length of distinct codes.
Given the set of all code streams $CS=\{cs_i~for~each~sequence~s_i\}$, the length of each type of code can be computed by Shannon entropy \cite{shannon1948mathematical}.
For pattern $p$, the length of the pattern code $code_p(p)$ is the negative log-likelihood
\begin{displaymath}
    L\left(code_p\left(p\right)\right)=-lg2\left(\frac{usage\left(p\right)}{\sum_{p_i \in CT}usage\left(p_i\right)}\right),
\end{displaymath}
where $lg2(k)$ means the logarithm of $k$ to the base $2$, and $usage(p)$ is the number of pattern codes of pattern $p$ in $CS$.
Similarly, we can give the calculation formulas for gap code $code_g(p)$, fill code $code_f(p)$, and miss code $code_m(p)$ as follows.
\begin{displaymath}
    \begin{aligned}
        L\left(code_g\left(p\right)\right)=&-lg2\left(\frac{gaps\left(p\right)}{gaps\left(p\right)+fills\left(p\right)+misses\left(p\right)}\right), \\
        L\left(code_f\left(p\right)\right)=&-lg2\left(\frac{fills\left(p\right)}{gaps\left(p\right)+fills\left(p\right)+misses\left(p\right)}\right), \\
        L\left(code_m\left(p\right)\right)=&-lg2\left(\frac{misses\left(p\right)}{gaps\left(p\right)+fills\left(p\right)+misses\left(p\right)}\right) \\ &+ L_N\left(~|~A~|~\right),
    \end{aligned}
\end{displaymath}
where $gaps(p)$, $fills(p)$, and $misses(p)$ are the number of gap codes, fill codes, and miss codes, respectively, of pattern $p$ in $CS$.
Miss code $code_m(p)$ contains additional bits for the index of missing attributes, which is denoted by $L_N(|A|)$.
Function $L_N(k)$ represents the number of bits required to encode integer $k$, where the MDL optimal Universal code for integers is considered \cite{grunwald2007minimum}.

\textbf{The encoded length of the code table.} To obtain a minimum description length, we treat patterns in $ST$ and patterns in $CT^*$ differently, where $L(CT~|~C)=L(ST)+L(CT^*)$.

For $ST$, we consider each attribute separately and encode the number of optional values and their supports:
\begin{displaymath}
    L\left(ST\right)=\sum_{1\leq k \leq ~|~A~|~}\left(L_N\left(~|~V_k~|~\right)
    + log\left(
        \begin{array}{c}
                ~|~S^k~|~ \\
                ~|~V_k~|~
            \end{array}
        \right)
    \right),
\end{displaymath}
where $S^k$ is a univariate dataset that preserves the $k$-th attribute of each event in dataset $S$.

For $CT^*$, we encode the number of patterns, the sum of their usages, the distribution of their usages over different patterns, and the original patterns:
\begin{displaymath}
    \begin{aligned}
        L\left(CT^*\right)= & L_N\left(~|~P^*~|~\right)+L_N\left(usage\left(P^*\right)\right)            \\
                            & +log\left(\begin{array}{c}
                ~|~usage\left(P^*\right)~|~ \\
                ~|~P^*~|~
            \end{array}\right)+\sum_{p_i\in P^*}L\left(p_i\right),
    \end{aligned}
\end{displaymath}
where $P^*$ is the set of all patterns in $CT^*$.
Considering that $|~P^*~|$ and $usage(P^*)$ can be zero, we define $L_N(0)=0$.
For a non-singleton pattern $p_i$, we encode the number of events, the number of values, the number of gaps, the number of misses, and the first column (i.e., each value in the pattern) as
\begin{displaymath}
    \begin{aligned}
        L\left(p_i\right) = & L_N\left(~|~p_i~|~\right)+L_N\left(~||~p_i~||~\right)                            \\
                            & +L_N\left(gaps\left(p_i\right)+1\right)+L_N\left(misses\left(p_i\right)+1\right) \\
                            & +\sum_{v\in p_i}L\left(code_p\left(v~|~ST\right)\right),
    \end{aligned}
\end{displaymath}
where $L(code_p(v ~|~ ST))$ represents the encoded length of a value $v$ in pattern $p_i$.
Here, we directly use the pattern code of singleton value $v$ in $ST$.

\textbf{The encoded length of the whole dataset given a code table.} We encode the number of sequences $|~S~|$, the length $|~s_i~|$ of each sequence $s_i$, the number of attributes $|~A~|$, and the codes in $CS$.
Thus, we obtain the equation
\begin{displaymath}
    \begin{aligned}
        L\left(S~|~CT\right)= & L_N\left(~|~S~|~\right) + \sum_{s_i \in S}L_N\left(~|~s_i~|~\right) + L_N\left(~|~A~|~\right) + L\left(CS\right),
    \end{aligned}
\end{displaymath}
where $L(CS)$ is the description length for $CS$ -- the sum of the description length of four types of codes:
\begin{displaymath}
    \begin{aligned}
        L\left(CS\right)= & \sum_{p_i \in CT}usage\left(p_i\right)L\left(code_p\left(p_i\right)\right)     \\
                          & + \sum_{p_i \in CT}gaps\left(p_i\right)L\left(code_g\left(p_i\right)\right)    \\
                          & + \sum_{p_i \in CT}fills\left(p_i\right)L\left(code_f\left(p_i\right)\right)   \\
                          & + \sum_{p_i \in CT}misses\left(p_i\right)L\left(code_m\left(p_i\right)\right).
    \end{aligned}
\end{displaymath}

==> archives/kdd2021/contents/3_4_problem.tex <==
\subsection{Problem Definition}

Before introducing our algorithm for obtaining the optimal model, we formally define our problem as follows.

\textbf{Optimal Pattern Set Problem.} \textit{Suppose that $A$ is a set of categorical attributes with finite values, and $S$ is a dataset of multivariate event sequences over these $|A|$ attributes. Find a set of multivariate patterns $P$ so that a cover $C$ of $S$ using $P$ can be found to obtain the minimum description length L(CT~|~C) + L(S~|~CT).}

For a problem like this, there exists a large search space, which leads to high runtime complexity.
First, because any subsequences of a sequence $s_i \in S$ can be a pattern, and thousands of sequences may exist, the set of patterns can be innumerable.
Second, given a set of patterns, we can cover $S$ in different ways.
We need to search for both the optimal set of patterns and the optimal way to cover the dataset.
When we introduce missing values, the search space becomes even larger. A pattern may not be a subsequence of any sequence in the dataset. And when using a pattern to cover a sequence, some values in the pattern may not necessarily appear in the sequence. In the next section, we explain how \textsc{Beep} can search this large space efficiently.


==> archives/kdd2021/contents/3_MDL.tex <==
\section{Basic Theory}

\label{sec:MDL}

In this section, we briefly introduce the Minimum Description Length (MDL) principle and how we apply it in sequence mining.

\input{contents/3_1_MDL.tex}
\input{contents/3_2_CT.tex}
\input{contents/3_3_Encoding.tex}
\input{contents/3_4_problem.tex}

==> archives/kdd2021/contents/4_1_Cover.tex <==
\subsection{Covering the Dataset}

\label{sec:coverAlgorithm}

Given a set of patterns $CT$ and a dataset $S$, the covering algorithm targets the optimal cover $C$ for each sequence $s_i \in S$ with the patterns in $CT$.
Considering that each sequence is independent, we cover the sequences separately.
Algorithm \ref{alg:cover} shows the process of obtaining the optimal cover $C$ given a sequence $s$ and patterns in $CT$.
First, we initialize three variables with an empty set (line 1), where $C$ is the output of the algorithm, $marks$ records which pattern each value in $s$ belongs to, and $misses$ records the position of all the miss values.
Note that $marks$ does not record any miss values, and $misses$ may record a value that is missed by two patterns.

The core idea is to traverse each pattern $p$ in $CT^*$ (line 2) and try to cover $s$ by $p$ (line 3\textasciitilde7) until all the values in $s$ are marked as covered by a pattern (line 8\textasciitilde9).
If there exist values not marked (line 10\textasciitilde12), they will be marked as covered by the corresponding singleton patterns in $ST$ (line 13\textasciitilde15).
To ensure that the final cover $C$ is optimal, we follow the \textsc{Krimp} algorithm \cite{vreeken2011krimp} and employ a greedy algorithm.
We traverse the patterns in $CT^*$ in a fixed order (Cover Order): $\downarrow ||~p~||$, $\downarrow support(p~|~S)$, and $\uparrow$ lexicographically.
This order ensures that the patterns that have more values and higher frequency, which are more meaningful, will be used first.
% To ensure that the final cover $C$ is optimal, we follow the \textsc{Krimp} algorithm \cite{vreeken2011krimp} and employ a greedy algorithm that traverses the patterns in $CT^*$ in a fixed order.
% We first consider patterns with more values, which are obviously more informative.
% We then consider patterns with higher frequency because higher frequency means more regularity.
% Finally, a lower likelihood of the cover are expected.
% Formally, the \textbf{Cover Order} is: $\downarrow ||~p~||$, $\downarrow support(p~|~S)$, and $\uparrow$ lexicographically.

Given a pattern $p$, a simple DFS-based algorithm (Appendix \ref{app:search}) searches pattern $p$ in sequence $s$ and finds every occurrence (line 3), where the limitations on gap events and missing values are considered.
For each time pattern where $p$ occurs, the searching algorithm returns the position of each value and the missing values, namely $marks_p$ and $misses_p$ respectively.
If all the positions in $marks_p$ are not marked, the algorithm uses pattern $p$ to cover these positions and updates the three variables.

\input{figures/a_covering.tex}

==> archives/kdd2021/contents/4_2_Summarize.tex <==
\subsection{Summarizing the Optimal Model}

\label{sec:summarizing}

Given a dataset $S$ and all singleton values in $ST$, the summarizing algorithm aims to find the optimal code table $CT$.
However, due to the large search space, finding the optimal $CT$ is time-consuming.
Inspired by \textsc{DITTO} \cite{bertens2016keeping}, we propose a heuristic algorithm to efficiently find an approximate optimal code table $CT$.
Algorithm \ref{alg:summarizing} demonstrates the algorithm overview.

The algorithm first initializes $CT$ with $ST$ (line 1).
Then a set of candidate patterns $Cand$ is generated (line 2) based on $S$ and $CT$.
The core idea of the algorithm is to examine whether each pattern $p$ in $Cand$ can bring information compression (line 3\textasciitilde4) and update $CT$ with $p$ that can do so (line 5\textasciitilde7).
To ensure priority access to a pattern that can bring higher information compression, the algorithm traverses the patterns $p$ in $Cand$ in the \textbf{Candidate Order}: $\downarrow support(p~|~S)$, $\downarrow |p|$, and $\uparrow$ lexicographically.

After confirming the ability of pattern $p$ to compress description length, the algorithm updates $CT$ with $p$ with three steps (line 5\textasciitilde7).
(1) The code table $CT$ is pruned to remove patterns that have become redundant with the addition of the new pattern $p$.
(2) The algorithm generates several variations of pattern $p$ to extend the code table efficiently.
(3) The algorithm updates the set of candidates for $CT$ based on the new code table $CT$.

We introduce three main functions below: the function for generating candidate patterns (Sec. \ref{sec:candidates}); the function for pruning (Sec. \ref{sec:pruning}); and the function for variations (Sec. \ref{sec:variations}).
We further introduce our method for speeding up the algorithm and the motivation for employing it (Sec. \ref{sec:lsh})

\input{algorithms/summarizing.tex}

\subsubsection{Generating Candidates}

\label{sec:candidates}

\input{figures/candidate}

A candidate pattern can be generated by combining two patterns that exist in $CT$, allowing us to construct complex patterns with simple ones.
Two patterns can be combined at different alignments.
To give the simplest example of univariate patterns, pattern $\{a, b\}$ and pattern $\{c, d\}$ can construct four candidates, namely, $\{a, b, c, d\}$, $\{a, c, b, d\}$, $\{c, a, d, b\}$, and $\{c, d, a, b\}$.
The combinations $\{a, c, d, b\}$ and $\{c, a, b, d\}$ are invalid because the number of gaps in $a, b$ and $c, d$ should be at most 1.
When constructing multivariate patterns, more candidates may arise, because the patterns may be related to different attributes such that the two patterns can be overlapped.
Furthermore, we need to consider the feature of missing values.
For example, in Fig. \ref{fig:candidate}, we list all the candidate patterns ($cp_1$ to $cp_6$) generated based on multivariate pattern $p_1$ and $p_2$ over three attributes.
When aligning the two events $e_2$ of $p_1$ and $p_2$, a conflict exists on value $x$ and $y$.
We resolve this conflict by regarding it as a missing value of one of the original patterns so that there exist two candidate patterns $cp_4$ and $cp_5$.
However, considering the limitation on the number of missing values, we regard these two candidates as invalid in practice.
We use $construct(p_i, p_j)$ to represent the set of all valid candidate patterns generated based on patterns $p_i$ and $p_j$.
We traverse each pair of patterns in $CT$ and construct candidate patterns.

% \input{algorithms/candidate}

\subsubsection{Pruning Patterns}

\label{sec:pruning}

If we add a new pattern $p^*$ into $CT$, some patterns may become redundant.
For example, if pattern $p_1={a}$ is always followed by pattern $p_2={b}$, all sequences containing $p_1$ can be covered by a new pattern $p^*={a,~b}$.
To keep the code table simple, we remove these redundant patterns.
Algorithm \ref{alg:pruning} demonstrates the process.
We first find all the patterns that have a lower usage after adding $p*$ (line 1\textasciitilde2).
Note that even if a singleton pattern has a lower support, we preserve it in $CT$ so that $CT$ always contains all singleton patterns.
Then, we traverse all the patterns to be pruned in \textbf{Prune Order}, where a pattern $p$ with a higher usage change $\Delta support(p)=usage(p~|~CT) - usage(p~|~CT_p)$ will be considered first.
If removing pattern $p$ can bring a smaller description length, we delete it from $CT$ (line 4\textasciitilde5).

\input{algorithms/pruning}

\subsubsection{Variations}

\label{sec:variations}

Constructing a large pattern is time-consuming, because we usually need to combine two patterns multiple times and examine all possible combinations.
To tackle this challenge, we follow the extremely effective solution used by \textsc{Ditto}: \textit{variations}.
The core idea of this algorithm is to quickly extend a pattern $p$ with the gap events that occur when using $p$ to cover the dataset.
More details can be found in Sec. 4.4 of \cite{bertens2016keeping}.

% \begin{algorithm}[t]
%     \caption{Function for Variations}
%     \label{alg:pruning}
%     \KwIn{The dataset $S$, a pattern $p^*$ and a code table $CT$}
%     \KwOut{A code table $CT$ with variations of $p$}
%     \tcc{the explanation can be found in Sec. \ref{sec:variations}}
%     $Cand \leftarrow p^* \times gapEvents(p^*)$\;
%     \For{{\bf each} $p \in Cand$}{
%         \If{$L(S,~CT \cup \{p\}) < L(S,~CT)$}{
%             $CT \leftarrow prune(S,~p,~CT) \cup \{p\}$\;
%             $CT \leftarrow variations(S,~p,~CT)$\;
%         }
%     }
%     \Return{$CT$}
% \end{algorithm}

\subsubsection{Speedup with Locality Sensitive Hashing (LSH)}

\label{sec:lsh}

The most time-consuming step was calculating the description length.
This is straightforward, as this was the only step that considered thousands of original sequences.
However, we found that, in line 4, Algorithm \ref{alg:summarizing}, a candidate $p$ is usually not an ideal pattern after comparing $L$, indicating that this step was wasting a lot of time examining useless candidates.
A faster algorithm would filter out those useless candidates before the description length step.

Since the candidate pattern is constructed from two patterns, when these two patterns often occur simultaneously or consecutively, the candidate pattern is more likely to be a real pattern.
Thus, we employ weighted \textit{Locality Sensitive Hashing} (LSH) \cite{ioffe2010improved} for efficiently determining whether two patterns can be combined.
If two sets of numbers have a weighted Jaccard similarity larger than a threshold $th$, the weighted LSH algorithm will generate the same hash value for them.

In our algorithm, for each pattern $p$, we record the positions where it occurs when covering the dataset.
A position is an index of a segment of original sequences, where a segment contains at most $l$ events (default $l$ is 20), and a long sequence will be cut into several segments.
If a pattern spans two segments, we record both positions.
Then we apply weighted LSH to examine whether the two patterns occur in similar sets of positions.
If the weighted LSH algorithm returns the same hash value, the candidate pattern constructed from these two patterns is indicated to be promising.

% 这里不太清楚是否需要加入一段，对应用MDL的内存消耗、时间消耗进行理论分析，还是只要最后进行实验就好了？
% Finally, we consider the runtime complexity and the memory requirements of LSH.
% Collecting the positions of a pattern in code table is not time-consuming.
% Before adding a pattern into code table, we have to computing the description length bases on the cover $C$ to examine whether the pattern brings information compression, where all the positions can be found $C$.


==> archives/kdd2021/contents/4_F4M.tex <==
\section{Algorithms}

\label{sec:F4M}

In this section, we introduce our algorithm, \textbf{BEEP}, to tackle the two challenges of covering the dataset and summarizing the optimal model.
The covering algorithm (Section \ref{sec:coverAlgorithm}) accepts the model summarized by the summarizing algorithm (Section \ref{sec:summarizing}) as input.
The summarizing algorithm optimizes the model iteratively according to the cover provided by the covering algorithm.

\input{contents/4_1_Cover.tex}
\input{contents/4_2_Summarize.tex}

==> archives/kdd2021/contents/5_RelatedWork.tex <==
\section{Related Work}

\label{sec:RelatedWork}

Over the decades, a number of sequential pattern mining algorithms, using a variety of different methods, have been built to analyze multivariate event sequences.

% SPM
Some traditional pattern mining algorithms use \textit{Breadth-First Search} (BFS) or \textit{Depth-First Search} (DFS) to search for patterns \cite{fournier2017survey}.
These algorithms require the number of occurrences of a pattern to be higher than a particular \textit{minimum support} threshold.
MSDD \cite{oates1996searching} was one of the first multivariate sequential pattern mining algorithms, and applied BFS to detect multi-stream dependency.
Tatti et al. \cite{tatti2011mining} presented an efficient BFS-based algorithm for discovering episodes with simultaneous events.
An algorithm by Wu et al. \cite{wu2013mining} assigned various levels of importance to different events that occurred simultaneously, in order to discover episodes with high utility.
TSKR \cite{morchen2007efficient} and CTMiner \cite{chen2010efficient} discovered patterns from datasets with interval-based events that might overlap.
All of these algorithms are susceptible to the well-known problem of \textit{pattern explosion} \cite{menger2015experimental} -- meaning that they return few patterns when the \textit{minimum support} is large, but a myriad of patterns when the threshold is loosened, making it challenging to determine the right threshold to obtain an appropriate number of patterns.

% MDL
Compared to more traditional pattern mining algorithms, MDL-based methods summarize a set of patterns to describe the entire sequence dataset instead of searching for each pattern, thus avoiding \textit{pattern explosion}.
Siebes et al. \cite{siebes2006item} first proposed applying the MDL principle to sequential pattern mining.
\textsc{Krimp} \cite{vreeken2011krimp} extended this theory and introduced a robust algorithm.
\textsc{Sqs} \cite{tatti2012long} defined an encoding scheme for finding serial episodes instead of itemsets.
Chen et al. \cite{chen2017sequence} and Deng et al. \cite{deng2019airvis} supported visual analytics and interactive exploration for the summarized patterns.
These algorithms, however, all worked for univariate sequence data.

% Multivariate
\textsc{Ditto} \cite{bertens2016keeping} first presented an MDL-based pattern mining algorithm for multivariate event sequences.
% however, \textsc{Ditto} cannot discover single-value noise.
\textsc{StreamScope} \cite{kawabata2018streamscope} was specifically designed to discover patterns in multi-dimensional data streams instead of static sequences.
Wu et al. \cite{wu2020visual} applied MDL to real-world applications and visualized multivariate patterns.
Compared with aforementioned multivariate pattern mining algorithm, our proposed method can handle single-value noises using a new encoding scheme.
Moreover, we employ an LSH-based acceleration to efficiently summarize patterns.

==> archives/kdd2021/contents/6_1_empirical.tex <==
\subsection{Empirical Study}

\subsubsection{Dataset}

To empirically evaluate the effectiveness of our algorithm, we conducted a case study on a real-world table tennis dataset.
Table tennis data is a typical example of multivariate event sequence data.
In table tennis singles matches, two players alternately hit the ball, beginning with one player's serve and ending with one player winning the game.
We considered each hit as an event and the consecutive hits as a sequence.
For each hit, we considered four attributes; namely, the technique the player used to hit the ball (\textit{Tech}), the area where the ball impacted the table (\textit{Ball}), the spin of the ball (\textit{Spin}), and the position of the player (\textit{Player}).
The optional values of these four attributes can be found in the Appendix \ref{app:values}.
We collected sequences from 10 matches (quarterfinals or later) played in 2019 by \textit{Ito Mima}, one of the top players in the world, against Chinese players.
We filtered sequences where \textit{Ito} served the ball in order to analyze her tactical patterns in this situation.
We were left with 716 sequences, of which the average length was 5.91.

\input{figures/caseTT}

\input{figures/t1_empirical.tex}

\subsubsection{Results analysis}

We ran both \textsc{Ditto} and \textsc{Beep} on this dataset and summarized the results (shown as Table \ref{tab:empirical}) as follows.

\textbf{\textsc{Beep} can summarize a smaller set of informative patterns than \textsc{Ditto}.}
\textsc{Beep} summarized 63 non-singleton patterns, while \textsc{Ditto} summarized 161.
According to the analysts we worked with, patterns with more than 4 values and used more than 10 times tend to be considered more worthy of analysis. Of these, \textsc{Beep} summarized 7 (used 530 times), while \textsc{Ditto} summarized 29 (used 546 times).
This was because many of the patterns that \textsc{Ditto} summarized as distinct differed in only one value, and \textsc{Beep} instead summarized these as one pattern with missing values.
As a result, \textsc{Beep} reduces the analysis burden of analysts.
Considering that the number of patterns is completely controlled by the algorithm, rather than manually input parameters, we believe that \textsc{Beep} is better than \textsc{Ditto} in summarizing a smaller set of informative patterns.

\textbf{\textsc{Beep} is more efficient than \textsc{Ditto} and performs similarly in information compression.}
We elaborate on these findings through quantitative experiments described in Section \ref{sec:quantitative}.

\subsubsection{Insights}

We discussed the summarized patterns with two analysts, each of whom has over three years of experience analyzing table tennis data for one of the best national teams in the world.
The patterns afforded the two analysts many insights into \textit{Ito}'s playing.
Due to space limitations, we'll focus here on one of the most common tactical patterns, shown as $p$ in Figure \ref{fig:tt}.

\input{figures/t2_quantitative.tex}

\textbf{\textsc{Beep} can find multivariate patterns that reveal the correlations among multiple attributes.}
In pattern $p$, \textit{Ito} first positioned herself at the \textit{Backhand} area and served with the \textit{Pendulum} technique.
Next, \textit{Ito}'s opponent stood at \textit{Backhand} and received the ball as it hit the table at the \textit{Short Backhand} position, using the control technique \textit{Push}.
Finally, \textit{Ito} stood at the \textit{Forehand} position and received the ball at \textit{Half-long Forehand} hitting with the technique \textit{Attack} and spinning type \textit{Sink}.
This pattern showed that \textit{Ito} preferred to use the attack technique at the third hit when her opponent used a control technique at the second hit.
At the same time, \textit{Ito} stood where she could hit the ball with her forehand, which results in a faster hit.
Furthermore, the \textit{Sink} spin made the ball lose height, giving her opponent less of a chance to return it well.
The analysts concluded that an excellent tactical pattern, which led to a high winning rate, benefits from various details.

\textbf{Missing values contribute to data analysis.}
The analysts found two sequences, $s_1$ and $s_2$ in Figure \ref{fig:tt}, that contain this pattern.
Sequence $s_1$ has a missing value at the second hit, where \textit{Ito}'s opponent used the technique \textit{Touch Short}, a control technique similar to \textit{Push}.
The analysts believed that $p$ summarized $s_1$ well, despite the missing value.
Sequence $s_2$ has a missing value at the third hit, where \textit{Ito} received the ball at \textit{Half-long Backhand}.
However, given that \textit{Ito} stood at the \textit{Forehand} area, it didn't seem possible for her to receive this ball.
The analysts checked the data and found this point to be an anomaly.
If we had instead used the \textsc{Ditto} algorithm, these two sequences would have been encoded by other short patterns and thus unable to reveal these insights.

% \subsubsection{ECG data}

% % data description
% ECG data consists of real-valued time series detected by sensors\footnote{physionet.org/physiobank/database/stdb}.
% Here we demonstrate how \textsc{Beep} discovers multivariate patterns in time series data.
% Since \textsc{Beep} only accepts event sequence data as input, we first need to transform the time series data into event sequence data.
% In our case, we chose two time series as detected by two sensors to construct a long sequence with two attributes.
% In order to discover patterns that could reveal overall characteristics, we sampled the two time so that every fifty real values were summarized by their average value.
% Next, we discretised the real values into categorical attributes by SAX \cite{lin2007experiencing}.
% Finally, we obtained a sequence of 10740 events with two attributes.
% Each attribute had five optional values.

% % insights
% \fillblank{A paragraph to describe insights}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{img/construct}
%     \caption{Examples for explaining how to construct candidate patterns. Given two patterns $p_1$ and $p_2$ over three attributes $a_1$ to $a_3$, .}
%     \Description{Summarizing two patterns from four sequences over two attributes.}
%     \label{fig:ecg}
% \end{figure}


==> archives/kdd2021/contents/6_2_quantitative.tex <==
\subsection{Quantitative Experiments}

\label{sec:quantitative}

\subsubsection{Synthetic data}

We performed quantitative experiments on multi-scaled synthetic data shown in Table \ref{tab:quantitative}.
We generated 15 datasets in 5 levels, varying in terms of the number of sequences ($|S|$), the length of each sequence ($|s_i|$), the number of attributes ($|A|$), and the number of optional values of each attribute ($|V_k|$).
The data generation consisted of three steps.
First, we generated sequences randomly, ensuring that all the optional values had similar frequencies.
More precisely, for any two optional values of an attribute, the frequency of one value must be higher than 90\% of the frequency of the other value.
Second, we generated 5 multivariate patterns, each of which contained 5 values and a random length.
Third, we added these patterns to the dataset generated in the first step.
We ensured that each pattern covered 10\% of the events in the dataset.
At the same time, for each pattern, we randomly chose two occurrences and set one value as a missing value for each occurrence, resulting in 10 total missing values.

\subsubsection{Experiments Setup}

We compared \textsc{Beep} with the state-of-art MDL-based multivariate pattern mining algorithm, \textsc{Ditto}, the source code of which has been implemented in C++ and published for research purposes\footnote{http://eda.mmci.uni-saarland.de/ditto/}.
Given that \textsc{Beep} mainly introduces two improvements -- namely, the miss codes and the LSH-based acceleration -- we performed an ablation study to evaluate how each improvement contributes to \textsc{Beep}.
Specifically, we considered five algorithms: (1) \textsc{Ditto}, (2) \textsc{Beep}-\,- (no miss codes; no LSH-based acceleration), (3) \textsc{Beep}-miss (no miss codes), (4) \textsc{Beep}-LSH (no LSH-based acceleration), and (5) the complete \textsc{Beep} algorithm.
Furthermore, we set the parameters of these algorithms, where the \textit{min support} of a pattern was $0.1 \times |S|$ for \textsc{Ditto}, and the threshold \textit{th} of LSH was $0.05 \times |S|$ for \textsc{Beep}-miss and \textsc{Beep}.
We ran the five algorithms on the 15 datasets and calculate the average performance of each algorithm on each level of datasets.

\subsubsection{Results}

The results are shown in Table \ref{tab:quantitative} and summarized as follows.

\textbf{\textsc{Beep} can discover all the planted patterns and missing values.} All five algorithms found all the planted patterns. Moreover, \textsc{Beep}-LSH and \textsc{Beep} detected all the planted missing values. Both \textsc{Ditto} and \textsc{Beep} work well in this scenario.

\textbf{\textsc{Beep}-\,- and \textsc{Ditto} have similar performance.} This proves that we can regard \textsc{Ditto} as the baseline algorithm and compare \textsc{Beep} with it fairly.

\textbf{LSH-based acceleration contributes to efficiency but sacrifices effectiveness.}
Comparing \textsc{Beep}-LSH with \textsc{Beep} and comparing \textsc{Beep}-\,- with \textsc{Beep}-miss, we find that LSH-based acceleration reduces runtime substantially.
However, when applying LSH-based acceleration, some patterns may not be found, meaning that the total description length may be longer.

\textbf{Miss codes help compress information but sacrifice efficiency.}
Comparing \textsc{Beep}-miss with \textsc{Beep} and comparing \textsc{Beep}-\,- with \textsc{Beep}-LSH, we find that miss codes can reduce the number of patterns and compress more information.
We believe that miss codes can filter out similar patterns and preserve only one, leaving a smaller set of meaningful patterns.
Miss codes also allow for the encoding of sequences with long patterns with missing values, rather than multiple short patterns, so that we obtain a short description length.
However, an algorithm that allows missing values spends more time searching for patterns.

\textbf{\textsc{Beep} strikes a good balance between effectiveness and efficiency.}
Comparing \textsc{Beep} with \textsc{Beep}-miss and \textsc{Beep}-LSH, we find that \textsc{Beep} balances the strengths of \textsc{Beep}-miss and \textsc{Beep}-LSH.
Although \textsc{Beep}-miss and \textsc{Beep}-LSH showed the best performance on efficiency and information compression, respectively, \textsc{Beep} has a nearly best performance on both efficiency and information compression.
In practice, analysts can choose one of these three algorithms according to their needs, although \textsc{Beep} will be the best choice in most scenarios.

==> archives/kdd2021/contents/6_Experiments.tex <==
\section{Experiments}

\label{sec:Experiments}

We implemented \textsc{Beep} in C++ and have open-sourced the code for research purposes\footnote{https://github.com/BEEP-algorithm/BEEP-algorithm}.
A computer with a 2 GHz CPU and 16 GB of memory was used in all experiments.
We first worked with analysts to conduct an empirical study on a real-world dataset, collecting their feedback on the number of patterns, the effectiveness of missing values, and the correlations among multiple attributes.
We further conducted quantitative experiments on multi-scaled synthetic datasets to compare \textsc{Beep} with the state-of-art multivariate pattern mining algorithm to evaluate the performance of \textsc{Beep}.

\input{contents/6_1_empirical.tex}
\input{contents/6_2_quantitative.tex}


==> archives/kdd2021/contents/7_Discussion.tex <==
\section{Discussion}

\label{sec:Discussion}

% significance
Through the case study on the real-world dataset, we empirically evaluated the effectiveness of \textsc{Beep}.
% The quantitative experiments on synthetic data show that \textsc{Beep} can strike a good balance between effectiveness and efficiency.
In practice, the analysts usually focused on the top five patterns, which had more events, more values, and higher support.
These patterns provided more insights into correlations among multiple attributes.
In the large dataset, \textsc{Beep} detected many missing values, where most missing values were substitutions of similar values and some were anomalies.
Thanks to the detection of missing values, some further studies could be conducted, such as analyzing the distribution of similar values, cleaning the data, and so on.

We quantitatively evaluated the efficiency of \textsc{Beep} through an ablation study on synthetic data. The results showed that the introduction of missing values could result in larger patterns and smaller description length, and that LSH-based acceleration could enhance runtime performance.
When both are employed, \textsc{Beep} strikes a good balance between effectiveness and efficiency.

% limitations:
% 1. different set of attributes for different events
% 2. different weight of different attributes
Through the analysts' feedback, we find two limitations.
First, some datasets may have different attributes in different events, such that correlations among attributes are more complicated.
For example, in soccer, the shooting angle is an essential attribute in a shooting event, but is useless in a passing event.
A possible solution is to assume each event has all attributes, and fill the irrelevant ones with empty values so that all events have the same attributes.
Second, some attributes may be more important for analysis, and could be assigned greater weights.
One possible solution for this is to give a longer code length to singletons of more important attributes, so that more non-singleton patterns related to these attributes can be summarized to compress the description.

% future work
% 1. interactive pattern mining
% 2. GPU acceleration
In the future, we plan to extend \textsc{Beep} for interactive pattern mining.
Although MDL considers the pattern set that minimizes the description length as the best, in practice, some ``best'' patterns cannot be explained by the analysts.
We expect an algorithm that can keep humans in the loop, so that analysts can interactively guide the algorithm to discover interpretable patterns.
Another future project could involve using GPU to accelerate the algorithm by running the covering and summarizing algorithms in parallel.

==> archives/kdd2021/contents/8_Conclusion.tex <==
\section{Conclusion}

\label{sec:Conclusion}

In this paper, we propose a novel encoding scheme to describe multivariate patterns in event sequence data.
Based on this encoding scheme, we can discover informative patterns that preserve correlations among multiple attributes and highlight any singleton noises in the dataset.
To efficiently surface these multivariate patterns from the original sequences, we propose \textsc{Beep}, an MDL-based heuristic algorithm made more efficient with LSH.
Through and empirical study on a real-world dataset and quantitative experiments on multi-scaled synthetic data, we prove that our algorithm strikes a good balance between effectiveness and efficiency.

==> archives/kdd2021/contents/9_acknowledgement.tex <==
\begin{acks}
...
\end{acks}

==> archives/kdd2021/contents/a_1_values.tex <==
\section{Optional values in the table tennis dataset}
\label{app:values}

There exist four attributes in the table tennis dataset.
All the optional values for each attribute are shown as Table \ref{tab:values}.

\begin{table}[!htb]
    \caption{The optional values of four attributes in the table tennis dataset.}
    \label{tab:values}
    \begin{tabular}{ll}
        \toprule

        Attributes&Optional values \\

        \midrule

        The technique used to hit   &Pendulum serving \\
        (16 optional values)        &Reverse serving \\
                                    &Tomahawk serving \\
                                    &Topspin \\
                                    &Smash \\
                                    &Attack \\
                                    &Flick \\
                                    &Twist \\
                                    &Push \\
                                    &Slide \\
                                    &Touch short \\
                                    &Block \\
                                    &Lob \\
                                    &Chopping \\
                                    &Pimpled techniques \\
                                    &Other techniques \\

        \cmidrule(lr){1-2}

        The area where the ball hit on the table    &Backhand serving \\
        (12 optional values)                        &Forehand serving \\
                                                    &Short forehand \\
                                                    &Half-long forehand \\
                                                    &Long forehand \\
                                                    &Short backhand \\
                                                    &Half-long backhand \\
                                                    &Long backhand \\
                                                    &Short middle \\
                                                    &Half-long middle \\
                                                    &Long middle \\
                                                    &Net or edge \\

        \cmidrule(lr){1-2}

        The type of ball's spinning &Strong topspin \\
        (7 optional values)         &Normal topspin \\
                                    &Strong downspin \\
                                    &Normal downspin \\
                                    &No spin \\
                                    &Sink \\
                                    &Without touching \\

        \cmidrule(lr){1-2}

        The position of the player  &Backhand serving \\
        (6 optional values)         &Forehand serving \\
                                    &Pivot \\
                                    &Backhand \\
                                    &Forehand \\
                                    &Back turn \\

        \bottomrule
    \end{tabular}
\end{table}

==> archives/kdd2021/contents/a_2_search.tex <==
\section{Search a pattern in a sequence}

\label{app:search}

Shown as Algorithm \ref{alg:search} and Algorithm \ref{alg:check}, we use a simple DFS to search all the occurrences of pattern $p$ in sequence $s$.

\begin{algorithm}[!htb]
    \caption{Searching Algorithm}
    \label{alg:search}
    \KwIn{A sequence $s$, a pattern $p$}
    \KwOut{All occurrences $occurs$}
    \tcc{the explanation can be found in Appendix \ref{app:search}}
    $occurs \leftarrow \emptyset$\;
    $max\_gaps \leftarrow |p| - 1$, $max\_misses \leftarrow (||p|| + 5) / 10$\;
    \For{$i \leftarrow$ 1 to $|s|$} {
        $found$, $marks$, $misses$ = dfs($s$, $p$, $i$, 1, $max\_gaps$, $max\_misses$)\;
        \If{$found$} {
            $occurs \leftarrow occurs + (marks, misses)$\;
        }
    }
    \Return{$occurs$}
\end{algorithm}

\begin{algorithm}[!htb]
    \caption{DFS Algorithm}
    \label{alg:check}
    \KwIn{A sequence $s$, a pattern $p$, the start index in sequence $si$, the start index in pattern $pi$, max number of gap events $max\_gaps$, max number of missing values $max\_misses$}
    \KwOut{Whether the patter occurs $found$, all positions $marks$, and positions of missing values $misses$}
    \tcc{the explanation can be found in Appendix \ref{app:search}}
    \If{$|s| - si < |p| - pi$} {
        \Return{{\bf false}}\;
    }

    $es \leftarrow$ the $si$-th event of $s$\;
    $ep \leftarrow$ the $pi$-th event of $p$\;
    $marks \leftarrow \emptyset$\;
    $num\_misses \leftarrow 0$, $misses \leftarrow \emptyset$\;
    \For{$k \leftarrow$ 1 to $|A|$} {
        \If{$ep[k]$ is not empty} {
            \eIf{$ep[k] != es[k]$} {
                $num\_misses += 1$\;
                $misses \leftarrow misses + (si, k)$
            } {
                $marks \leftarrow marks + (si, k)$
            }
        }
    }
    \If{$num_misses > max_misses$} {
        \Return{{\bf false}}\;
    }

    \For{$i \leftarrow 0$ to $max\_gaps$} {
        $found$, $marks^*$, $misses^*$ = dfs($s$, $p$, $si+1+i$, $pi+1$, $max\_gaps-i$, $max\_misses-num\_misses$)\;
        \If{$found$} {
            $marks \leftarrow marks \cup marks^*$\;
            $misses \leftarrow misses \cup misses^*$\;
            \Return{{\bf true}, marks, misses}\;
        }
    }
    \Return{{\bf false}}\;
\end{algorithm}

==> archives/kdd2021/contents/t1_empirical.tex <==
\begin{table}
    \caption{The results of the empirical study on the table tennis data. We compared two algorithms, namely \textsc{Ditto} and \textsc{Beep}, on the number of patterns ($|P|$), the average length of non-singleton patterns (\textit{$avg.$} $|p_i|$), the gain in compression compared to the singleton-only model ($\Delta L\%$), the number of missing values ($miss$, only for \textsc{Beep}), and the runtime ($t$).}
    \label{tab:empirical}
    \begin{tabular}{rrrrrr}
        \toprule

        % $|S|$&\textit{avg.} $|s_i|$&$|A|$&$|E|$ &
        \textit{Algorithm}   &   $|P|$    &   \textit{avg.} $|p_i|$   &    $\Delta L\%$    &    $miss$   &   $t$(s) \\

        \midrule

        \textsc{Ditto} & 161 & 4.17 & 55.38 & -- & 1747 \\

        \textsc{Beep} & 62 & 3.65 & 47.03& 280 & 425 \\

        \bottomrule
    \end{tabular}
\end{table}

==> archives/kdd2021/contents/t2_quantitative.tex <==
\begin{table*}
    \caption{The results of the quantitative experiments. Given 5 synthetic datasets, one for each row, we compared five algorithms, namely, \textsc{Ditto}, \textsc{Beep}-\,-, \textsc{Beep}-miss, \textsc{Beep}-LSH, and \textsc{Beep}. For each dataset, we reported the number of sequences ($|S|$), the number of events in each sequence ($|s_i|$), the number of attributes ($|A|$), and the number of optional values of each attribute ($|V_k|$). For each algorithm, we reported the number of patterns ($|P|$), the gain in compression compared to the singleton-only model ($\Delta L\%$), the number of missing values for \textsc{Beep}-LSH and \textsc{Beep} ($miss$), and the runtime in seconds ($t$). (\tablet{orange}: the shortest time; \tabledL{blue}: the largest gain in information compression.)}
    \label{tab:quantitative}
    \begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
      \toprule

      \multicolumn{4}{l}{Synthetic Datasets}&\multicolumn{3}{l}{\textsc{Ditto}}&\multicolumn{3}{l}{\textsc{Beep}-\,-}&\multicolumn{3}{l}{\textsc{Beep}-miss}&\multicolumn{4}{l}{\textsc{Beep}-LSH}&\multicolumn{4}{l}{\textsc{Beep}} \\

      \cmidrule(lr){1-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-17}\cmidrule(lr){18-21}

      $|S|$&  $|s_i|$&      $|A|$&  $|V_k|$&
      $|P|$&  $\Delta L\%$& $t$(s)&
      $|P|$&  $\Delta L\%$& $t$(s)&
      $|P|$&  $\Delta L\%$& $t$(s)&
      $|P|$&  $\Delta L\%$& $miss$& $t$(s)&
      $|P|$&  $\Delta L\%$& $miss$& $t$(s) \\

      \midrule

      50& 20& 5& 100&
      19&   24.5&     399&
      19&   24.5&     380&
      16&   24.4&     \tablet{43}&
      9&   \tabledL{27.2}&     33&455&
      9&   \tabledL{27.2}&     33& 79\\

      \textbf{70}& 20& 5& 100&
      12&   19.0&     987&
      12&   19.0&     994&
      12&   18.9&     \tablet{29}&
      14&   \tabledL{21.3}&     16&1238&
      14&   \tabledL{21.3}&     11& 215\\

      50& \textbf{30}& 5& 100&
      20&   25.8&     772&
      20&   25.8&     753&
      20&   25.9&     \tablet{120}&
      14&   \tabledL{26.7}&     29& 1276&
      13&   26.6&     28& 402\\

      50& 20& \textbf{7}& 100&
      15&   27.7&     1040&
      15&   27.7&     1028&
      14&   27.7&     \tablet{43}&
      9&   \tabledL{29.2}&     31& 1141&
      9&   29.1&     30& 251\\

      50& 20& 5& \textbf{200}&
      17&   24.1&     175&
      17&   24.1&     168&
      16&   24.1&     19&
      10&   25.2&     39& 149&
      9&   \tabledL{25.3}&     39& \tablet{18}\\

      \bottomrule
    \end{tabular}
  \end{table*}

==> archives/kdd2021/figures/candidate.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/construct}
    \caption{Examples for explaining how to construct candidate patterns. Given two patterns $p_1$ and $p_2$ over three attributes $a_1$ to $a_3$, we construct six candidate patterns $cp_1$ to $cp_6$ at different alignments. Candidates $cp_4$ and $cp_5$ demonstrate how we fix a conflict by missing values.}
    \Description{Summarizing two patterns from four sequences over two attributes.}
    \label{fig:candidate}
\end{figure}

==> archives/kdd2021/figures/caseTT.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/caseTT}
    \caption{Patterns found in table tennis data. Two sequences $s_1$ and $s_2$ contain pattern $p$ (highlighted in blue) and have missing values (highlighted in red).}
    \Description{Summarizing two patterns from four sequences over two attributes.}
    \label{fig:tt}
\end{figure}

==> archives/kdd2021/figures/encoding.tex <==
\begin{figure}[!tp]
    \centering
    \includegraphics[width=\linewidth]{img/encoding}
    \caption{Examples for explaining the process of encoding. Given sequence $s$ and code table $CT$, we first obtain the cover $C$, where sequence $s$ is described by the patterns in $CT$. We further obtain the code stream $CS$, where sequence $s$ is encoded by the four types of codes in $CT$.}
    \Description{Summarizing two patterns from four sequences over two attributes.}
    \label{fig:ct}
\end{figure}

==> archives/kdd2021/figures/patternDefinition.tex <==
\begin{figure}[!tp]
  \centering
  \includegraphics[width=\linewidth]{img/patternDefinition}
  \caption{Examples for explaining the definition of patterns. The dataset consists of four sequences ($s_1$ to $s_4$) and considers two attributes ($a_1$ and $a_2$). We summarize two patterns ($p_1$ and $p_2$).}
  \Description{Summarizing two patterns from four sequences over two attributes.}
  \label{fig:patterndef}
\end{figure}

==> figures/a_candidate.tex <==
\begin{algorithm}[t]
    \caption{Function for Candidate Patterns}
    \label{alg:candidate}
    \KwIn{A code table $CT$}
    \KwOut{A candidate code table $Cand$}
    \tcc{the explanation can be found in Sec. \ref{sec:candidates}}
    \For{{\bf each} $p_i \in CT$}{
        \For{{\bf each} $p_j \in CT$}{
            $Cand \leftarrow Cand \cup construct(p_i,~p_j)$\;
        }
    }
    \Return{$Cand$}
\end{algorithm}

==> figures/a_covering.tex <==
\begin{algorithm}[t]
    \caption{Covering Algorithm}
    \label{alg:cover}
    \KwIn{A sequence $s$, a code table $CT$}
    \KwOut{An optimal cover $C$}
    \tcc{the explanation can be found in Sec. \ref{sec:coverAlgorithm}}
    $C \leftarrow \emptyset$, $marks \leftarrow \emptyset$, $misses \leftarrow \emptyset$\;
    \For{{\bf each} $p\in CT^*$ in Cover Order} {
        \For{{\bf each} $(marks\_p, misses\_p) \in search(p, s)$}{
            \If{$marks \cap marks\_p = \emptyset$}{
                $C \leftarrow C \cup (marks\_p, misses\_p)$\;
                $marks \leftarrow marks \cup marks\_p$\;
                $misses \leftarrow misses \cup misses\_p$\;
            }
        }
        \If{$|marks| = |s| \times |A|$}{
            {\bf break}\;
        }
    }
    \For{{\bf each} event $e \in s$} {
        \For{{\bf each} value $v \in e$} {
            \If{$v$ is not marked by $marks$} {
                $mark$ = \{cover $v$ by singleton pattern $v$ in $ST$\}\;
                $C \leftarrow C \cup (mark, \emptyset)$\;
                $marks \leftarrow marks \cup mark$\;
            }
        }
    }
    \Return{$C$}
\end{algorithm}

==> figures/a_pruning.tex <==
\begin{algorithm}[t]
    \caption{Function for Pruning}
    \label{alg:pruning}
    \KwIn{The dataset $S$, a new pattern $p^*$, and a code table $CT$}
    \KwOut{A pruned code table $CT$}
    \tcc{the explanation can be found in Sec. \ref{sec:pruning}}
    $CT_p = CT \cup \{p^*\}$\;
    $PruneCand = \{p\in CT^*~|~usage(p~|~CT_p)<usage(p~|~CT)\}$\;
    \For{{\bf each} $p \in PruneCand$ in Prune Order}{
        \If{$L(S,~CT \setminus p) < L(S,~CT)$}{
            $CT \leftarrow CT \setminus p$\;
        }
    }
    \Return{$CT$}
\end{algorithm}

==> figures/a_summarizing.tex <==
\begin{algorithm}[t]
    \caption{Summarizing Algorithm}
    \label{alg:summarizing}
    \KwIn{The dataset $S$ and the standard code table $ST$}
    \KwOut{An approximate optimal code table $CT$}
    \tcc{the explanation can be found in Sec. \ref{sec:summarizing}}
    $CT \leftarrow ST$\;
    $Cand \leftarrow candidate(CT)$\;
    \For{{\bf each} $p \in Cand$ in Candidate Order}{
        \If{$L(S,~CT \cup \{p\}) < L(S,~CT)$}{
            $CT \leftarrow prune(S,~p,~CT) \cup \{p\}$\;
            $CT \leftarrow variations(S,~p,~CT)$\;
            $Cand \leftarrow candidate(CT)$\;
        }
    }
    \Return{$CT$}
\end{algorithm}
